Leveraging Allophony in Self-Supervised Speech Models for Atypical Pronunciation Assessment

Allophony refers to the variation in the phonetic realization of a phoneme based on its phonetic environment. Modeling allophones is crucial for atypical pronunciation assessment, which involves distinguishing atypical from typical pronunciations. However, recent phoneme classifier-based approaches often simplify this by treating various realizations as a single phoneme, bypassing the complexity of modeling allophonic variation. Motivated by the acoustic modeling capabilities of frozen self-supervised speech model (S3M) features, we propose MixGoP, a novel approach that leverages Gaussian mixture models to model phoneme distributions with multiple subclusters. Our experiments show that MixGoP achieves state-of-the-art performance across four out of five datasets, including dysarthric and non-native speech. Our analysis further suggests that S3M features capture allophonic variation more effectively than MFCCs and Mel spectrograms, highlighting the benefits of integrating MixGoP with S3M features.

==> figures/tab_melspec.tex <==
\begin{table*}[t]
\caption{
Kendall-tau correlation coefficient between the pronunciation scores and the dysfluency/disfluency (absolute value).
Bigger is better.
}
\label{tab:melspec}
\vspace{0.5em}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccc|cccc}
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Feature} & \multicolumn{4}{c|}{Phoneme classification} & \multicolumn{4}{c}{Phoneme density modeling} \\
\cmidrule{3-6} \cmidrule{7-10}
 & & GMM- & NN- & DNN- & MaxLogit- & kNN & oSVM & p-oSVM & MixGoP \\
  & & GoP & GoP & GoP & GoP &  &  &  & (Proposed) \\
 % & & \citep{Witt2000PhonelevelPS} & \citep{hu2015improved} & \citep{hu2015improved} & \citep{yeo23_interspeech} & \citep{sun2022out} & \citep{scholkopf2001estimating,shahin2023phonological} & \citep{scholkopf2001estimating} & (Ours) \\
\midrule
UASpeech
& MelSpec & 0.2093 & 0.1718 & 0.2422 & 0.2141 & 0.1012 & 0.0993 & 0.0863 & 0.0394 \\
\midrule
TORGO
& MelSpec & 0.2707 & 0.2619 & 0.1497 & 0.2711 & 0.2869 & 0.2114 & 0.2405 & 0.1959 \\
\midrule
SSNCE
& MelSpec & 0.1828 & 0.1609 & 0.0513 & 0.1869 & 0.1537 & 0.1139 & 0.1064 & 0.1739 \\
\midrule
speechocean762
& MelSpec & 0.2135 & 0.0641 & 0.2318 & 0.2290 & 0.1111 & 0.1090 & 0.0709 & 0.0038 \\
\midrule
L2-ARCTIC
& MelSpec & 0.0491 & 0.0389 & 0.0319 & 0.0319 & 0.0222 & 0.0034 & 0.0269 & 0.0103 \\
\bottomrule
\end{tabular}%
}
\end{table*}

